HyDA-Vista: Towards Optimal Guided Selection of k-mer Size for Sequence Assembly

Motivation: Intimately tied to assembly quality is the complexity of the de Bruijn graph built by the assembler. Thus, there have been many paradigms developed to decrease the complexity of the de Bruijn graph. One obvious combinatorial paradigm for this is to allow the value of $k$ to vary; having a larger value of $k$ where the graph is more complex and a smaller value of $k$ where the graph would likely contain fewer spurious edges and vertices. One open problem that affects the practicality of this method is how to predict the value of $k$ prior to building the de Bruijn graph. We show that optimal values of $k$ can be predicted prior to assembly by using the information contained in a phylogenetically-close genome and therefore, help make the use of multiple values of $k$ practical for genome assembly. Results: We present HyDA-Vista, which is a genome assembler that uses homology information to choose a value of $k$ for each read prior to the de Bruijn graph construction. The chosen $k$ is optimal if there are no sequencing errors and the coverage is sufficient. Fundamental to our method is the construction of the {\em maximal sequence landscape}, which is a data structure that stores for each position in the input string, the largest repeated substring containing that position. In particular, we show the maximal sequence landscape can be constructed in $O(n + n \log n)$-time and $O(n)$-space. HyDA-Vista first constructs the maximal sequence landscape for a homologous genome. The reads are then aligned to this reference genome, and values of $k$ are assigned to each read using the maximal sequence landscape and the alignments. Eventually, all the reads are assembled by an iterative de Bruijn graph construction method. Our results and comparison to other assemblers demonstrate that HyDA-Vista achieves the best assembly of {\em E. coli} before repeat resolution or scaffolding.

==> footer.tex <==


\section*{Acknowledgement}
Text Text Text Text Text Text  Text Text.  \citealp{Boffelli03} might want to know about  text text text text

\paragraph{Funding\textcolon} Text Text Text Text Text Text  Text Text.

%\bibliographystyle{natbib}
%\bibliographystyle{achemnat}
%\bibliographystyle{plainnat}
%\bibliographystyle{abbrv}

\bibliography{document.bib}
%\bibliographystyle{bioinformatics}

\bibliographystyle{plain}

==> methods.tex <==
HyDA-Vista involves three stages: construction of the maximal sequence landscape, assignment of $k$-mers to reads, and de Bruijn graph assembly.  An overview of HyDA-Vista is shown in Algorithm \ref{alg:hyda}.  We explain each of these steps in detail in the subsequent subsections. %The MCL-WMR algoforithm first chooses a {\em reference sequence} from the data set, denoted as $S_r$, building the entire graph from all the input data (including $S_r$), and for each vertex $v_{r \gamma}$ representing the $l$-length subsequence from $S_r$ starting at position $\gamma$.  We then use MCL to generate subgraphs which contain vertices that are highly inter-related, from these clusters of vertices we will generate the positions of the possible motif instances and their corresponding motif consensus. The algorithm terminates when a motif is found.  In order to increase the probability a motif is found, we minimize searching subgraphs with low probability of containing a motif; hence, the adjacency subgraphs are not clustered and searched in a sequential manner.

\begin{algorithm*}[h]
\caption{An overview of HyDA-Vista}
\label{alg:hyda}
\begin{algorithmic}[1]
\State  Build the maximal sequence landscape for the reference genome.
\State  Align all reads to the reference using BWA.
\State  For each aligned read: assign a value of $k$ using the maximal sequence landscape.
\State  Unaligned reads are assigned a value of $k$ using a heuristic.
\State  The de Bruijn graph is constructed in an iterative manner. 
\end{algorithmic}
\end{algorithm*}
